Chiron: A Robust Recommendation System with Graph Regularizer

Recommendation systems have been widely used by commercial service providers for giving suggestions to users. Collaborative filtering (CF) systems, one of the most popular recommendation systems, utilize the history of behaviors of the aggregate user-base to provide individual recommendations and are effective when almost all users faithfully express their opinions. However, they are vulnerable to malicious users biasing their inputs in order to change the overall ratings of a specific group of items. CF systems largely fall into two categories - neighborhood-based and (matrix) factorization-based - and the presence of adversarial input can influence recommendations in both categories, leading to instabilities in estimation and prediction. Although the robustness of different collaborative filtering algorithms has been extensively studied, designing an efficient system that is immune to manipulation remains a significant challenge. In this work we propose a novel "hybrid" recommendation system with an adaptive graph-based user/item similarity-regularization - "Chiron". Chiron ties the performance benefits of dimensionality reduction (through factorization) with the advantage of neighborhood clustering (through regularization). We demonstrate, using extensive comparative experiments, that Chiron is resistant to manipulation by large and lethal attacks.

==> bibliography.tex <==
@article{Koren09matrixfactorization,
 author = {Koren, Yehuda and Bell, Robert and Volinsky, Chris},
 title = {Matrix Factorization Techniques for Recommender Systems},
 journal = {Computer},
 issue_date = {August 2009},
 volume = {42},
 number = {8},
 month = aug,
 year = {2009},
 issn = {0018-9162},
 pages = {30--37},
 numpages = {8},
 url = {http://dx.doi.org/10.1109/MC.2009.263},
 doi = {10.1109/MC.2009.263},
 acmid = {1608614},
 publisher = {IEEE Computer Society Press},
 address = {Los Alamitos, CA, USA},
 keywords = {Computational intelligence, Computational intelligence, Netflix Prize, Matrix factorization, Matrix factorization, Netflix Prize},
}

@article{DBLP:journals/corr/JungL13a,
  author    = {Hyun Joon Jung and
               Matthew Lease},
  title     = {Crowdsourced Task Routing via Matrix Factorization},
  journal   = {CoRR},
  volume    = {abs/1310.5142},
  year      = {2013},
  timestamp = {Mon, 04 Nov 2013 15:55:47 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/JungL13a},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{journals/debu/MehtaH08,
  author = {Mehta, Bhaskar and Hofmann, Thomas},
  date = {2008-07-01},
  description = {dblp},
  journal = {IEEE Data Eng. Bull.},
  number = 2,
  pages = {14-22},
  title = {A Survey of Attack-Resistant Collaborative Filtering Algorithms.},
  volume = 31,
  year = 2008
}

@INPROCEEDINGS{Bennett07thenetflix,
    author = {James Bennett and Stan Lanning and Netflix Netflix},
    title = {The Netflix Prize},
    booktitle = {In KDD Cup and Workshop in conjunction with KDD},
    year = {2007}
}

@inproceedings{Lawrence:2009:NMF:1553374.1553452,
 author = {Lawrence, Neil D. and Urtasun, Raquel},
 title = {Non-linear Matrix Factorization with Gaussian Processes},
 booktitle = {Proceedings of the 26th Annual International Conference on Machine Learning},
 series = {ICML '09},
 year = {2009},
 isbn = {978-1-60558-516-1},
 location = {Montreal, Quebec, Canada},
 pages = {601--608},
 numpages = {8},
 publisher = {ACM},
 address = {New York, NY, USA},
} 


@inproceedings{Mehta:2007:USD:1619797.1619870,
 author = {Mehta, Bhaskar},
 title = {Unsupervised Shilling Detection for Collaborative Filtering},
 booktitle = {Proceedings of the 22Nd National Conference on Artificial Intelligence - Volume 2},
 series = {AAAI'07},
 year = {2007},
 isbn = {978-1-57735-323-2},
 pages = {1402--1407},
 numpages = {6},
 acmid = {1619870},
 publisher = {AAAI Press},
} 


@inproceedings{Zhang:2006:ALL:1148170.1148259,
 author = {Zhang, Sheng and Ouyang, Yi and Ford, James and Makedon, Fillia},
 title = {Analysis of a Low-dimensional Linear Model Under Recommendation Attacks},
 booktitle = {Proceedings of the 29th Annual International ACM SIGIR Conference on Research and Development in Information Retrieval},
 series = {SIGIR '06},
 year = {2006},
 isbn = {1-59593-369-7},
 pages = {517--524},
 numpages = {8},
 acmid = {1148259},
 publisher = {ACM},
 address = {New York, NY, USA},
} 



@inproceedings{Cosley:2003:SBR:642611.642713,
 author = {Cosley, Dan and Lam, Shyong K. and Albert, Istvan and Konstan, Joseph A. and Riedl, John},
 title = {Is Seeing Believing? How Recommender System Interfaces Affect Users' Opinions},
 booktitle = {Proceedings of the SIGCHI Conference on Human Factors in Computing Systems},
 series = {CHI '03},
 year = {2003},
 isbn = {1-58113-630-7},
 location = {Ft. Lauderdale, Florida, USA},
 pages = {585--592},
 numpages = {8},
 acmid = {642713},
 publisher = {ACM},
 address = {New York, NY, USA},
} 


@inproceedings{Salakhutdinov:2008:BPM:1390156.1390267,
 author = {Salakhutdinov, Ruslan and Mnih, Andriy},
 title = {Bayesian Probabilistic Matrix Factorization Using Markov Chain Monte Carlo},
 booktitle = {Proceedings of the 25th International Conference on Machine Learning},
 series = {ICML '08},
 year = {2008},
 isbn = {978-1-60558-205-4},
 location = {Helsinki, Finland},
 pages = {880--887},
 numpages = {8},
 doi = {10.1145/1390156.1390267},
 acmid = {1390267},
 publisher = {ACM},
 address = {New York, NY, USA},
} 


@ARTICLE{6980102, 
author={Niemann, K. and Wolpers, M.}, 
journal={Learning Technologies, IEEE Transactions on}, 
title={Creating Usage Context-based Object Similarities to Boost Recommender Systems in Technology Enhanced Learning}, 
year={2014}, 
month={}, 
volume={PP}, 
number={99}, 
pages={1-1}, 
keywords={Context;Equations;Frequency measurement;Portals;Recommender systems;Semantics;Vectors;Learning Analytics;Learning Web Portals;Recommender Systems;Technology Enhanced Learning;Web Mining}, 
doi={10.1109/TLT.2014.2379261}, 
ISSN={1939-1382},}

@inproceedings{lee2013local,
  added-at = {2013-11-19T00:00:00.000+0100},
  author = {Lee, Joonseok and Kim, Seungyeon and Lebanon, Guy and Singer, Yoram},
  biburl = {http://www.bibsonomy.org/bibtex/2f0ad51071d16332b1069d4ff08ad003d/dblp},
  booktitle = {ICML (2)},
  crossref = {conf/icml/2013},
  ee = {http://jmlr.org/proceedings/papers/v28/lee13.html},
  interhash = {3031746ef3cfbf8c845104628b3bd062},
  intrahash = {f0ad51071d16332b1069d4ff08ad003d},
  keywords = {dblp},
  pages = {82-90},
  publisher = {JMLR.org},
  series = {JMLR Proceedings},
  timestamp = {2015-04-28T15:24:53.000+0200},
  title = {Local Low-Rank Matrix Approximation.},
  url = {http://dblp.uni-trier.de/db/conf/icml/icml2013.html#LeeKLS13},
  volume = 28,
  year = 2013
}


@article{Resnick:2008:MRS:1486877.1486887,
  added-at = {2010-01-19T00:00:00.000+0100},
  author = {Resnick, Paul and Sami, Rahul},
  biburl = {http://www.bibsonomy.org/bibtex/2c3781cc763c07fdc605f638f9834bd4e/dblp},
  date = {2010-01-19},
  description = {dblp},
  ee = {http://doi.acm.org/10.1145/1486877.1486887},
  interhash = {bec1fb20b847a85573d2f1d40f2b739a},
  intrahash = {c3781cc763c07fdc605f638f9834bd4e},
  journal = {SIGecom Exchanges},
  keywords = {dblp},
  number = 3,
  timestamp = {2010-01-20T11:36:00.000+0100},
  title = {Manipulation-resistant recommender systems through influence limits.},
  url = {http://dblp.uni-trier.de/db/journals/sigecom/sigecom7.html#ResnickS08},
  volume = 7,
  year = 2008
} 


@inproceedings{Lam:2004:SRS:988672.988726,
 author = {Lam, Shyong K. and Riedl, John},
 title = {Shilling Recommender Systems for Fun and Profit},
 booktitle = {Proceedings of the 13th International Conference on World Wide Web},
 series = {WWW '04},
 year = {2004},
 isbn = {1-58113-844-X},
 location = {New York, NY, USA},
 pages = {393--402},
 numpages = {10},
 doi = {10.1145/988672.988726},
 acmid = {988726},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {collaborative filtering, recommender systems, shilling},
} 

@inproceedings{Bhattacharjee:2007:AIR:1283383.1283428,
 author = {Bhattacharjee, Rajat and Goel, Ashish},
 title = {Algorithms and Incentives for Robust Ranking},
 booktitle = {Proceedings of the Eighteenth Annual ACM-SIAM Symposium on Discrete Algorithms},
 series = {SODA '07},
 year = {2007},
 isbn = {978-0-898716-24-5},
 location = {New Orleans, Louisiana},
 pages = {425--433},
 numpages = {9},
 acmid = {1283428},
 address = {Philadelphia, PA, USA},
} 

@inproceedings{Chirita:2005:PSA:1097047.1097061,
 author = {Chirita, Paul-Alexandru and Nejdl, Wolfgang and Zamfir, Cristian},
 title = {Preventing Shilling Attacks in Online Recommender Systems},
 booktitle = {Proceedings of the 7th Annual ACM International Workshop on Web Information and Data Management},
 series = {WIDM '05},
 year = {2005},
 isbn = {1-59593-194-5},
 location = {Bremen, Germany},
 pages = {67--74},
 numpages = {8},
 doi = {10.1145/1097047.1097061},
 acmid = {1097061},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {collaborative filtering, recommender systems, shilling attacks, web applications},
} 

@INPROCEEDINGS{Belkin01laplacianeigenmaps,
    author = {Mikhail Belkin and Partha Niyogi},
    title = {Laplacian Eigenmaps and Spectral Techniques for Embedding and Clustering},
    booktitle = {Advances in Neural Information Processing Systems 14},
    year = {2001},
    pages = {585--591},
    publisher = {MIT Press}
}


@INPROCEEDINGS{OMahony06detectingnoise,
   author = {O'Mahony, Michael P. and Hurley, Neil J. and Silvestre, Gu{\'e}nol{\'e} C.M.},
 title = {Detecting Noise in Recommender System Databases},
 booktitle = {Proceedings of the 11th International Conference on Intelligent User Interfaces},
 series = {IUI '06},
 year = {2006},
 isbn = {1-59593-287-9},
 location = {Sydney, Australia},
 pages = {109--115},
 numpages = {7},
 url = {http://doi.acm.org/10.1145/1111449.1111477},
 doi = {10.1145/1111449.1111477},
 acmid = {1111477},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@article{Mobasher:2007:TTR:1278366.1278372,
 author = {Mobasher, Bamshad and Burke, Robin and Bhaumik, Runa and Williams, Chad},
 title = {Toward Trustworthy Recommender Systems: An Analysis of Attack Models and Algorithm Robustness},
 journal = {ACM Trans. Internet Technol.},
 issue_date = {October 2007},
 volume = {7},
 number = {4},
 month = oct,
 year = {2007},
 issn = {1533-5399},
 articleno = {23},
 doi = {10.1145/1278366.1278372},
 acmid = {1278372},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {Profile injection attacks, attack detection, collaborative filtering, recommender systems, shilling},
} 


@inproceedings{Mehta:2008:ARC:1390334.1390350,
 author = {Mehta, Bhaskar and Nejdl, Wolfgang},
 title = {Attack Resistant Collaborative Filtering},
 booktitle = {Proceedings of the 31st Annual International ACM SIGIR Conference on Research and Development in Information Retrieval},
 series = {SIGIR '08},
 year = {2008},
 isbn = {978-1-60558-164-4},
 location = {Singapore, Singapore},
 pages = {75--82},
 numpages = {8},
 doi = {10.1145/1390334.1390350},
 acmid = {1390350},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {SVD, collaborative filtering, recommendation algorithm, shilling},
} 


@incollection{omahony2002,
year={2002},
booktitle={Database and Expert Systems Applications},
volume={2453},
series={Lecture Notes in Computer Science},
title={Promoting Recommendations: An Attack on Collaborative Filtering},
publisher={Springer Berlin Heidelberg},
author={O'Mahony, MichaelP. and Hurley, NeilJ. and Silvestre, GuenoleC.M.},
pages={494-503},
}

@incollection{NIPS2014_5537,
title = {A Statistical Decision-Theoretic Framework for Social Choice},
author = {Azari Soufiani, Hossein and Parkes, David C and Xia, Lirong},
booktitle = {Advances in Neural Information Processing Systems 28},
series = {NIPS '14},
pages = {3185--3193},
year = {2014},
}

@incollection{NIPS2003_2506,
title = {Learning with Local and Global Consistency},
author = {Zhou, Denny and Olivier Bousquet and Thomas N. Lal and Weston, Jason and Sch\"{o}lkopf, Bernhard},
booktitle = {Advances in Neural Information Processing Systems 16},
editor = {S. Thrun and L. K. Saul and B. Sch\"{o}lkopf},
pages = {321--328},
year = {2004},
publisher = {MIT Press},
url = {http://papers.nips.cc/paper/2506-learning-with-local-and-global-consistency.pdf}
}

@Inbook{Zheng2016,
author="Zheng, Jing
and Liu, Jian
and Shi, Chuan
and Zhuang, Fuzhen
and Li, Jingzhi
and Wu, Bin",
editor="Bailey, James
and Khan, Latifur
and Washio, Takashi
and Dobbie, Gill
and Huang, Joshua Zhexue
and Wang, Ruili",
title="Dual Similarity Regularization for Recommendation",
bookTitle="Advances in Knowledge Discovery and Data Mining: 20th Pacific-Asia Conference, PAKDD 2016, Auckland, New Zealand, April 19-22, 2016, Proceedings, Part II",
year="2016",
publisher="Springer International Publishing",
address="Cham",
pages="542--554",
isbn="978-3-319-31750-2",
doi="10.1007/978-3-319-31750-2_43",
url="http://dx.doi.org/10.1007/978-3-319-31750-2_43"
}


@article{citeulike:14072193,
    author = {Wang, Yixin and Kucukelbir, Alp and Blei, David M.},
    citeulike-article-id = {14072193},
    citeulike-linkout-0 = {http://arxiv.org/pdf/1606.03860.pdf},
    keywords = {bayes\_theorem, bayesian, bayesian\_inference, blei\_dm, graphical\_models, probability, robustness},
    posted-at = {2016-06-20 00:18:11},
    priority = {2},
    title = {{Reweighted Data for Robust Probabilistic Models}},
    url = {http://arxiv.org/pdf/1606.03860.pdf}
}


@Inbook{Guan2016,
author="Guan, Xin
and Li, Chang-Tsun
and Guan, Yu",
editor="Bailey, James
and Khan, Latifur
and Washio, Takashi
and Dobbie, Gill
and Huang, Joshua Zhexue
and Wang, Ruili",
title="Enhanced SVD for Collaborative Filtering",
bookTitle="Advances in Knowledge Discovery and Data Mining: 20th Pacific-Asia Conference, PAKDD 2016, Auckland, New Zealand, April 19-22, 2016, Proceedings, Part II",
year="2016",
publisher="Springer International Publishing",
address="Cham",
pages="503--514",
isbn="978-3-319-31750-2",
doi="10.1007/978-3-319-31750-2_40",
url="http://dx.doi.org/10.1007/978-3-319-31750-2_40"
}

@incollection{NIPS2007_1007,
    address = {Cambridge, MA},
    author = {Salakhutdinov, Ruslan and Mnih, Andriy},
    booktitle = {Advances in Neural Information Processing Systems 20},
    citeulike-article-id = {2147262},
    editor = {Platt, J. C. and Koller, D. and Singer, Y. and Roweis, S.},
    keywords = {bibtex-import, matrix-factorization},
    posted-at = {2007-12-19 16:14:13},
    priority = {5},
    publisher = {MIT Press},
    title = {{Probabilistic Matrix Factorization}},
    year = {2008}
}


@online{movielens,
  note = {MovieLens \url{http://grouplens.org/datasets/movielens/}
}


@article{DBLP:journals/corr/AgarwalA0NT13,
  author    = {Alekh Agarwal and
               Animashree Anandkumar and
               Prateek Jain and
               Praneeth Netrapalli and
               Rashish Tandon},
  title     = {Learning Sparsely Used Overcomplete Dictionaries via Alternating Minimization},
  journal   = {CoRR},
  volume    = {abs/1310.7991},
  year      = {2013},
  url       = {http://arxiv.org/abs/1310.7991},
  timestamp = {Mon, 04 Nov 2013 15:55:49 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/AgarwalA0NT13},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@INPROCEEDINGS{Joachims03transductivelearning,
    author = {Thorsten Joachims},
    title = {Transductive learning via spectral graph partitioning},
    booktitle = {In ICML},
    year = {2003},
    pages = {290--297}
}


@ARTICLE{Cai11GNMF,
         AUTHOR = {Deng Cai and Xiaofei He and Jiawei Han and Thomas S. Huang},
         TITLE = {Graph Regularized Non-negative Matrix Factorization for Data Representation},
         JOURNAL = {IEEE Transactions on Pattern Analysis and Machine Intelligence},
         YEAR = {2011},
         volume = {33},
         number = {8},
         pages = {1548-1560}, 
}

@article{Belkin:2006:MRG:1248547.1248632,
 author = {Belkin, Mikhail and Niyogi, Partha and Sindhwani, Vikas},
 title = {Manifold Regularization: A Geometric Framework for Learning from Labeled and Unlabeled Examples},
 journal = {J. Mach. Learn. Res.},
 issue_date = {12/1/2006},
 volume = {7},
 month = dec,
 year = {2006},
 issn = {1532-4435},
 pages = {2399--2434},
 numpages = {36},
 url = {http://dl.acm.org/citation.cfm?id=1248547.1248632},
 acmid = {1248632},
 publisher = {JMLR.org},
} 


@inproceedings{conf/nips/SoufianiPX12,
  added-at = {2014-12-10T00:00:00.000+0100},
  author = {Soufiani, Hossein Azari and Parkes, David C. and Xia, Lirong},
  booktitle = {Advances in Neural Information Processing Systems 26},
  series = {NIPS '12},
  crossref = {conf/nips/2012},
  pages = {126-134},
  title = {Random Utility Theory for Social Choice.},
  year = 2012
}

@incollection{NIPS2013_4998,
  added-at = {2014-01-07T00:00:00.000+0100},
  author = {Soufiani, Hossein Azari and Diao, Hansheng and Lai, Zhenyu and Parkes, David C.},
  biburl = {http://www.bibsonomy.org/bibtex/24c99b0658f130a45bb5fa2ab16ebf6cb/dblp},
  booktitle = {Advances in Neural Information Processing Systems 27},
  series = {NIPS '13},
  crossref = {conf/nips/2013},
  ee = {http://papers.nips.cc/paper/4998-generalized-random-utility-models-with-multiple-types},
  interhash = {6a3a9c97f0eecba59e13157b3e74b5c9},
  intrahash = {4c99b0658f130a45bb5fa2ab16ebf6cb},
  keywords = {dblp},
  pages = {73-81},
  timestamp = {2015-04-28T14:19:20.000+0200},
  title = {Generalized Random Utility Models with Multiple Types.},
  url = {http://dblp.uni-trier.de/db/conf/nips/nips2013.html#SoufianiDLP13},
  year = 2013
}

@inproceedings{chaney2015probabilistic,
  title={A probabilistic model for using social networks in personalized item recommendation},
  author={Chaney, Allison JB and Blei, David M and Eliassi-Rad, Tina},
  booktitle={Proceedings of the 9th ACM Conference on Recommender Systems},
  pages={43--50},
  year={2015},
  organization={ACM}
}

@book{citeulike:7047477,
    author = {Rasch, G.},
    citeulike-article-id = {7047477},
    editor = {Press, M. E. S. A.},
    isbn = {0-941938-05-0},
    keywords = {rasch},
    posted-at = {2010-04-21 11:18:09},
    priority = {2},
    publisher = {MESA Press},
    title = {{Probabilistic Models for Some Intelligence and Attainment Tests.}},
    year = {1960}
}


@article{lee99,
    author = {Lee, Daniel D. and Seung, H. Sebastian},
    citeulike-article-id = {83540},
    citeulike-linkout-0 = {http://dx.doi.org/10.1038/44565},
    citeulike-linkout-1 = {http://dx.doi.org/10.1038/401788a0},
    citeulike-linkout-2 = {http://view.ncbi.nlm.nih.gov/pubmed/10548103},
    citeulike-linkout-3 = {http://www.hubmed.org/display.cgi?uids=10548103},
    day = {21},
    doi = {10.1038/44565},
    issn = {0028-0836},
    journal = {Nature},
    keywords = {feature, nlp-reading, semantic},
    month = oct,
    number = {6755},
    pages = {788--791},
    pmid = {10548103},
    posted-at = {2006-05-05 05:40:02},
    priority = {0},
    publisher = {Nature Publishing Group},
    title = {{Learning the parts of objects by non-negative matrix factorization}},
    url = {http://dx.doi.org/10.1038/44565},
    volume = {401},
    year = {1999}

}

@incollection{NIPS2000_1861,
title = {Algorithms for Non-negative Matrix Factorization},
author = {Daniel D. Lee and H. Sebastian Seung},
booktitle = {Advances in Neural Information Processing Systems 13},
series = {NIPS '01},
pages = {556--562},
year = {2001},
publisher = {MIT Press},
}


@inproceedings{conf/flairs/SeminarioW12,
  added-at = {2012-07-11T00:00:00.000+0200},
  author = {Seminario, Carlos E. and Wilson, David C.},
  biburl = {http://www.bibsonomy.org/bibtex/2f9d0484563923a79d43ea3abc290b5ec/dblp},
  booktitle = {FLAIRS Conference},
  crossref = {conf/flairs/2012},
  ee = {http://www.aaai.org/ocs/index.php/FLAIRS/FLAIRS12/paper/view/4418},
  interhash = {f40c2f47d12baa5e46210f8af993ba40},
  intrahash = {f9d0484563923a79d43ea3abc290b5ec},
  isbn = {978-1-57735-558-8},
  keywords = {dblp},
  publisher = {AAAI Press},
  timestamp = {2012-07-12T11:33:26.000+0200},
  title = {Robustness and Accuracy Tradeoffs for Recommender Systems Under Attack.},
  url = {http://dblp.uni-trier.de/db/conf/flairs/flairs2012.html#SeminarioW12},
  year = 2012}


@inproceedings{citeulike:4563135,
    author = {Paterek, Arkadiusz},
    booktitle = {Proc. KDD Cup Workshop at SIGKDD'07, 13th ACM Int. Conf. on Knowledge Discovery and Data Mining},
    location = {San Jose, CA, USA},
    pages = {39--42},
    title = {{Improving regularized singular value decomposition for collaborative filtering}},
    year = {2007}
}


@inproceedings{Burke:2006:CFA:1150402.1150465,
 author = {Burke, Robin and Mobasher, Bamshad and Williams, Chad and Bhaumik, Runa},
 title = {Classification Features for Attack Detection in Collaborative Recommender Systems},
 booktitle = {Proceedings of the 12th ACM SIGKDD International Conference on Knowledge Discovery and Data Mining},
 series = {KDD '06},
 year = {2006},
 location = {Philadelphia, PA, USA},
 pages = {542--547},
 numpages = {6},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@MISC{Jansen03ananalysis,
    author = {Bernard J Jansen and Amanda Spink},
    title = {An Analysis of Web Documents Retrieved and Viewed},
    year = {2003}
}
@inproceedings{Resnick:1994:GOA:192844.192905,
 author = {Resnick, Paul and Iacovou, Neophytos and Suchak, Mitesh and Bergstrom, Peter and Riedl, John},
 title = {GroupLens: An Open Architecture for Collaborative Filtering of Netnews},
 booktitle = {Proceedings of the 1994 ACM Conference on Computer Supported Cooperative Work},
 series = {CSCW '94},
 year = {1994},
 isbn = {0-89791-689-1},
 location = {Chapel Hill, North Carolina, USA},
 pages = {175--186},
 numpages = {12},
 url = {http://doi.acm.org/10.1145/192844.192905},
 doi = {10.1145/192844.192905},
 acmid = {192905},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {Usenet, collaborative filtering, electronic bulletin boards, information filtering, netnews, selective dissemination of information, social filtering, user model},
} 

@article{rashid2005irb,
  added-at = {2007-11-21T16:03:11.000+0100},
  author = {Rashid, A. M. and Karypis, G. and Riedl, J.},
  biburl = {http://www.bibsonomy.org/bibtex/265e6a92489e5190ca5129532d2d138fd/wnpxrz},
  interhash = {9fcc40d7537a7d10df92a3e2effb8f69},
  intrahash = {65e6a92489e5190ca5129532d2d138fd},
  journal = {Proceedings of the SIAM International Conference on Data Mining},
  keywords = {recommendersystems},
  timestamp = {2007-11-21T16:03:11.000+0100},
  title = {{Influence in ratings-based recommender systems: An algorithm-independent approach}},
  url = {http://www.grouplens.org/papers/pdf/RashidAl_siam05.pdf},
  year = 2005
}

@paper{seminario2012,
	author = {Carlos Seminario and David Wilson},
	title = {Robustness and Accuracy Tradeoffs for Recommender Systems Under Attack},
	conference = {Florida Artificial Intelligence Research Society Conference},
	year = {2012}
}

@article{Koren:2009:MFT:1608565.1608614,
 author = {Koren, Yehuda and Bell, Robert and Volinsky, Chris},
 title = {Matrix Factorization Techniques for Recommender Systems},
 journal = {Computer},
 issue_date = {August 2009},
 volume = {42},
 number = {8},
 month = aug,
 year = {2009},
 issn = {0018-9162},
 pages = {30--37},
 numpages = {8},
 acmid = {1608614},
 publisher = {IEEE Computer Society Press},
 address = {Los Alamitos, CA, USA},
} 

@article{Lee:2012:PPR:2503308.2503328,
 author = {Lee, Joonseok and Sun, Mingxuan and Lebanon, Guy},
 title = {PREA: Personalized Recommendation Algorithms Toolkit},
 journal = {J. Mach. Learn. Res.},
 issue_date = {January 2012},
 volume = {13},
 number = {1},
 month = sep,
 year = {2012},
 issn = {1532-4435},
 pages = {2699--2703},
 numpages = {5},
 acmid = {2503328},
 publisher = {JMLR.org},
} 

@inproceedings{conf/camsap/BoydSR15,
  added-at = {2016-01-28T00:00:00.000+0100},
  author = {Boyd, Nicholas and Schiebinger, Geoffrey and Recht, Benjamin},
  biburl = {http://www.bibsonomy.org/bibtex/2c8c20ab7152db5d9d601dace965b1e10/dblp},
  booktitle = {CAMSAP},
  crossref = {conf/camsap/2015},
  ee = {http://dx.doi.org/10.1109/CAMSAP.2015.7383735},
  interhash = {cf1dfc3006a2615d581003e0233506e1},
  intrahash = {c8c20ab7152db5d9d601dace965b1e10},
  isbn = {978-1-4799-1963-5},
  keywords = {dblp},
  pages = {57-60},
  publisher = {IEEE},
  timestamp = {2016-01-29T11:46:06.000+0100},
  title = {The alternating descent conditional gradient method for sparse inverse problems.},
  url = {http://dblp.uni-trier.de/db/conf/camsap/camsap2015.html#BoydSR15},
  year = 2015
}



@ARTICLE{2012arXiv1205.3193L,
  author    = {Joonseok Lee and
               Mingxuan Sun and
               Guy Lebanon},
  title     = {A Comparative Study of Collaborative Filtering Algorithms},
  journal   = {CoRR},
  volume    = {abs/1205.3193},
  year      = {2012},
  url       = {http://arxiv.org/abs/1205.3193},
  timestamp = {Wed, 10 Oct 2012 21:28:52 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/abs-1205-3193},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@Article{optimisationavecconstraint1969,
    Author = {A. {Auslender}},
    Title = {{M\'ethodes du second ordre dans les probl\`emes d'optimisation avec contraintes.}},
    Journal = {{Rev. Fran\c{c}. Inform. Rech. Op\'er.}},
    Volume = {3},
    Number = {R-2},
    Pages = {27--42},
    Year = {1969},
    Publisher = {Association Fran\c{c}aise d'Informatique et de Recherche Op\'erationnelle (AFIRO), Paris},
    Language = {French}
 }
